Learning to Identify Perceptual Bugs in 3D Video Games

Automated Bug Detection (ABD) in video games is composed of two distinct but complementary problems: automated game exploration and bug identification. Automated game exploration has received much recent attention, spurred on by developments in fields such as reinforcement learning. The complementary problem of identifying the bugs present in a player's experience has for the most part relied on the manual specification of rules. Although it is widely recognised that many bugs of interest cannot be identified with such methods, little progress has been made in this direction. In this work we show that it is possible to identify a range of perceptual bugs using learning-based methods by making use of only the rendered game screen as seen by the player. To support our work, we have developed World of Bugs (WOB) an open platform for testing ABD methods in 3D game environments.

==> temp.tex <==

%In our setting, testing tools are operating at a higher level of abstraction. Comprised of a software agent, the agent aims to get good code coverage (now called environment coverage) by taking the actions available too it, as a human player would, to explore the game environment. When doing so, it may encounter issues similar to those found at a lower level in the form of program crashes/errors. However at this higher level there is a new fundamentally different kind of bug that manifests. As an unfortunate side effect of the way modern engines perform error handling, these bugs often fail \textit{silently}. They tend also to be difficult to write conditions for and so are not caught by standard developer error handling code. Fig. \ref{fig:BugHierarchy} gives the hierarchy of bugs, the ones of interest, at least for this work are those that lie at the boundary of automation. Logical bugs include issues with the physics engine, typically as part of complex interactions between objects or components, progression/narrative related issues or information related issues, such as the player obtaining information before they are supposed to. Visual bugs are usually a result of an issue with the rendering system, but also include any bug that changes what the player should other wise see, these may include issues with the games physics. \todo{what is a behavioural bug...}. There is some overlap between the levels present, in that visual, logical and behavioural bugs can sometimes be caught by developer code by circumventing much of the complexity involved. In fact, much of the work on automated bug identification has focused on ways to write conditions that deal with bugs at this level, on specifying the relationships between different game components and conditions for verifying their state \todo{cite}. These approaches are time consuming to implement, require extensive knowledge of the interactions, and do not address the classic problem of limited imagination on the part of the developer. There has also been work on automatically identifying visual bugs. In some limited settings, like for simple mobile games, it is possible to write conditions and rely on simple vision based methods\cite{Mozgovoy2018, Tuovenen2019}, but the richness of the presentation in many video games makes this in general impractical. 

%At the highest levels of abstraction, it is widely agreed that conditions for bug identification cannot be practically specified\todo{}\cite{}. This is the level at which human game testers operate, their job is to explore the game (by playing) and to identify bugs that have either been overlooked by the developer (in that they could have error checking conditions, but don't) or those in which the developer was not practically able to specify conditions. The game tester uses their knowledge of how the game is \textit{supposed} to behave, a high-level specification, and their vast experience, both in game and in the real world to determine whether a particular encounter is valid or not. Notice that the game tester does both exploration (game playing) \textit{and} identification and that they are to some extent distinct. As it turns out, an experienced game tester will direct their exploration towards areas in which they feel they are more likely to identify a bug, this relationship between exploration and identification with regard to the automation of both has not been explored in any depth in the ADB literature, but is one that we feel will become increasingly important. Some recent work has recognised the connection and makes use of data from human testers to guide the exploration \cite{Ariyurek2021}.

%Our focus is on a collection of visual bugs that are not game specific, our hope is that progress on these bugs will not only be useful for the broadest audience but that progress here will transfer to some bugs that are game specific. Visual bugs are also perhaps the easiest to address as they generally don't require high-level knowledge of the intended behaviour (such as knowledge about the games narrative, progression, etc). The collection of visual bugs we consider are related to the interaction between two very complex programs that form the majority of a fully fledged game engine - the physics engine, and the rendering pipeline.  Both programs are typically written by specialist and made available to developers via some kind of (reasonably) high-level API. The developers of these programs cannot anticipate their specific use and are general, in the sense that they any error checking cannot be game/application specific. Our platform has implemented a number of these complex visual bugs, one instructive example is camera clipping. 

%For efficiency reasons, geometry in a game scene is culled, removing anything that is out of the view. One version of this is called frustum culling, which culls geometry that lies outside of the camera frustum (a box that defines what the camera can see in the 3D space). The the side of the frustum closest to the camera is called the near clipping plane, if any geometry is too close to the camera (behind the near clipping plane) it will be culled, this is to prevent objects getting too close and causing issues with the final screen projection. However, while avoiding one issue, it introduces another. The player may be able to see inside objects, or through walls if the near clipping plane is not \textit{near enough}. This may give players information that should otherwise not be able to access, is visually undesirable and breaks immersion. It is extremely difficult to write conditions to identify a clipping issue for a complex level geometry, particularly when dynamic objects are involved. Various tricks are used in practice to avoid the problem, but they are not foolproof.

%A more sophisticated mechanism is required to detect these kinds of bugs, one that is more similar to the trusty game tester. In fact, this has already been recognised on the exploration side \todo{cite}. Researchers are developing more sophisticated agents that are closer to human players/game testers than traditional more traditional rule/search based systems. The incorporation of learning into these agents has become a key tool in allowing them to explore more effectively. We are advocating that systems that learn from experience will also be required for the identification problem, especially if there is to be progress in the highest levels of abstraction. The \acr\ platform is a step in this direction as it supports researchers in training and testing their approaches in both exploration and identification.  the 
\todo{grab citations for this section.}
